A General Framework for Adversarial Examples with Objectives

Images perturbed subtly to be misclassified by neural networks, called adversarial examples, have emerged as a technically deep challenge and an important concern for several application domains. Most research on adversarial examples takes as its only constraint that the perturbed images are similar to the originals. However, real-world application of these ideas often requires the examples to satisfy additional objectives, which are typically enforced through custom modifications of the perturbation process. In this paper, we propose adversarial generative nets (AGNs), a general methodology to train a generator neural network to emit adversarial examples satisfying desired objectives. We demonstrate the ability of AGNs to accommodate a wide range of objectives, including imprecise ones difficult to model, in two application domains. In particular, we demonstrate physical adversarial examples---eyeglass frames designed to fool face recognition---with better robustness, inconspicuousness, and scalability than previous approaches, as well as a new attack to fool a handwritten-digit classifier.

==> app-alg-agn.tex <==
\section{\agn{} Training Algorithm}
\label{app:agn_alg}

\algref{alg:agn} presents a psuedocode the algorithm for
training \agn{}s (see \secref{sec:framework} for a description).

%%%%%%%% alg %%%%%%%%
\begin{algorithm}
  \small
 \caption{\agn{} training}\label{alg:agn}

  \SetKwData{Left}{left}\SetKwData{This}{this}\SetKwData{Up}{up}
  \SetKwFunction{Union}{Union}\SetKwFunction{FindCompress}{FindCompress}
  \SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}

  \Input{$X$, \gen{}, \discrim{}, \dnnFunc{}, $\mathit{dataset}$, $Z$, $N_e$, $s_b$, 
	$\kappa \in \{0,1\}$}
  \Output{Adversarial \gen{}}
  \BlankLine
  $e\leftarrow 0$\;
  \For{$e\leftarrow 1$ \KwTo $N_e$~}{
      create $\varname{mini-batches}$ of size $s_b$ from $\mathit{dataset}$\;
      \For{$\mathit{batch}$ $\in$ $\varname{mini-batches}$}{
        $z\leftarrow s_b$ samples from $Z$\;
        $\mathit{gen}\leftarrow G(z)$\;
        $\mathit{batch}$$\leftarrow$ $\mathit{concat(gen, batch)}$\;
        \If(\tcp*[h]{update \discrim}){even iteration}{
            update \discrim{} by backpropagating $\frac{\partial \Gain_{D}}{\partial batch}$\;
        }\Else(\tcp*[h]{update \gen}){
            \lIf{\dnnFunc{} fooled}{
               return
            }
            $d_1\leftarrow -\frac{\partial \Gain_{D}}{\partial gen}$\;
            $x\leftarrow s_b$ sample images from $X$\;
            $x\leftarrow x + gen$\;
            Compute forward pass $F(x)$\;
            $d_2\leftarrow \frac{\partial \Loss_{F}}{\partial gen}$\;
            $d_1, d_2 \leftarrow normalize(d_1, d_2)$\;
            $d \leftarrow \kappa \cdot d_1 + (1-\kappa) \cdot d_2$\;
            update \gen{} via backpropagating $d$\;
        }
      }
  }
\end{algorithm}
%%%%%%%% End alg %%%%%%%%


==> app-architectures.tex <==
\section{DNN Architectures}
\label{app:archs}

\tabref{fig:dnn_archs} summarizes the architectures we used for the
generator and discriminator in \agns{}, as well as of the DNNs we
attacked and the detector we used; these are discussed in \secref{sec:attack-impl}.

\input{tables/architectures}


==> app-result-mnist.tex <==
\section{\agn{}s Against Digit Recognition}
\label{app:mnist}

\figref{fig:mnist} illustrates samples from the 5,004 adversarial
examples generated via \agn{}s to fool the digit-recognition \dnn{}. The adversarial
examples were produced by first generating 600,000 images using the adversarial
generators (60,000 per generator). Out of all samples, 8.34\% of samples that
were misclassified by the \dnn{} were kept. Out of these, only the digits that were
likely to be comprehensible by humans were kept: the filtration process involved
computing the product of the discriminator's output (i.e., how realistic the images
were deemed by the discriminator) and the probability assigned by the digit-recognition
\dnn{} to the correct class, and keeping the 10\% of digits with the highest product.

% figure %
\begin{figure}[tbh]
\centering
\includegraphics[width=42pt]{figures/mnist-samples.jpg}\hspace{12pt}
\includegraphics[width=42pt]{figures/mnist-pretrained-gen-samples.jpg}\hspace{12pt}
\includegraphics[width=42pt]{figures/mnist-untargeted-adv-examples.jpg}
\caption{An illustration of attacks generated via \agn{}s. Left: A random sample
	of digits from MNIST. Middle: Digits generated by the pretrained generator.
	Right: Digits generated via \agn{}s that are misclassified by the digit-recognition
	\dnn{}.}
\label{fig:mnist}
\end{figure}


==> app-result-transfer.tex <==
\section{Transferability of Dodging Attacks}
\label{app:sec:transfer}

In this section, we explore whether dodging against \dnn{}s of one architecture
leads to successful dodging against \dnn{}s of a different architecture. Indeed,
the transferability of attacks has been shown to be effective in fooling models to
which adversaries do not have access (e.g.,~\cite{Papernot17Blackbox}). In our
case, although this is not an explicit goal of our attacks, attackers with access to
one \dnn{} but not another may attempt to rely on transferability to dodge against
the second \dnn{}.

% table %
\input{tables/transfer.tex}

Using the data from \secref{sec:digital}, we first tested whether
dodging in the digital environment successfully transferred between
architectures (see \tabref{tab:transfer_digital}). We found that
attacks against the OpenFace architecture successfully fooled the VGG
architecture in only a limited number of attempts (10--12\%). In
contrast, dodging against VGG led to successful dodging against
OpenFace in at least 63.33\% of attempts.

Universal attacks seemed to transfer between architectures with
similar success.  Using attacks created with 100 subjects and 10
eyeglasses from \secref{sec:universal}, we found that about 81.54\%
($\pm 2.82\%$ standard deviation) of attacks transferred from \vggL{}
to \openfaceL{}, and 26.15\% ($\pm 3.94\%$ standard deviation)
transferred in the other direction.

As opposed to dodging in the digital environment, physically realized
dodging attacks do not transfer well (see
\tabref{tab:transfer_physical}). Using the frames that successfully
dodged from \secref{sec:real}, we found that none of the video frames
that successfully dodged against the OpenFace \dnn{}s managed to dodge
against the VGG \dnn{}s, and only a small percentage (7--18\%) of the
video frames that dodged against VGG, successfully dodged against
OpenFace.


==> app-result-univ-dodge.tex <==
\section{Universal Dodging Results}
\label{app:universal}

\algref{alg:universal} presents a psuedocode of the algorithm
used to generate universal eyeglasses for different clusters of
users, as described in~\secref{sec:universal}.

\input{universal-algorithm.tex}


\figref{app:fig:universal} shows the results of universal dodging both
against \vggL{} and \openfaceL{}; these are discussed in \secref{sec:universal}.

\begin{figure}[t]
	\centering
	% VGG143 universal
	\begin{subfigure}[b]{0.49\textwidth}
		\centering
		\includegraphics[width=0.98\columnwidth]{figures/universal-vgg143-thin.pdf}
	\caption{Universal dodging against \vggL{}.}\label{fig:vgg_univ}
	\end{subfigure}
	% OpenFace143 universal
	\begin{subfigure}[b]{0.49\textwidth}
		\centering
		\includegraphics[width=0.98\columnwidth]{figures/universal-openface143-thin.pdf}
                \caption{Universal dodging against \openfaceL{}.}
	\label{fig:openface_univ}
	\end{subfigure}
	% caption
	\caption{Universal dodging against \vggL{} and \openfaceL{}. The x-axis shows
		the number of subjects used to train the adversarial generators. When the number of
		subjects is zero, a non-adversarial generator was used. The y-axis shows the mean fraction
		of images misclassified (i.e., the dodging success rate). The whiskers on the
		bars show the standard deviation of the success rate, computed by repeating each
		experiment five times, each time with a different set of randomly picked subjects. The
		color of the bars denotes the number of eyeglasses used, as shown in the legend.
		We evaluated each attack
		using one, two, five, or ten eyeglasses. For example,
                the rightmost bar in \figref{fig:openface_univ}
                indicates that an \agn{} trained with images of 100
                subjects will generate eyeglasses such that 10 pairs
                of eyeglasses will allow approximately 94\% of
                subjects to evade recognition.
		For $\le 10$ subjects, \algref{alg:agn} was used
		to create the attacks.
                For 50 and 100 subjects, \algref{alg:universal}
		was used.}
	\label{app:fig:universal}
\end{figure}


==> discussion.tex <==
\section{Discussion}
\label{sec:discuss}

\agns{} provide a general methodology to train a generator neural
network to emit adversarial examples that satisfy desired objectives.
They are especially useful when meeting objectives, such as
inconspicuousness, that may elude precise specification. In principle, given
an objective that can be described through a set of examples, \agn{}s
can be trained to emit adversarial examples that satisfy this objective.

We demonstrated the \agn{}s are general enough to craft successful
attacks in the context of face and digit recognition. We expect that they
would generalize to other applications, as well. For example, one may
consider using \agn{}s to fool \dnn{}s for street-sign recognition by training
the generator to emit adversarial examples that resemble
street-sign images collected from the internet.

We found that \agn{}s, in addition to achieving more objectives, craft physical
domain attacks that are more inconspicuous and robust than prior work
that considered a similar threat model~\cite{Sharif16AdvML}. Thus, \agn{}s
are important to consider when evaluating the resilience of machine-learning
algorithms against attacks in the physical domain.

One advantage of \agn{}s over other attack methods
(e.g.,~\cite{Szegedy13NNsProps,Gdfllw14ExpAdv}) is that they can
generate more than one adversarial example for a given benign sample.
A diverse set of adversarial examples can be useful for evaluating
the robustness of models. Moreover, such adversarial examples may be
used to defend against attacks (e.g., by incorporating them in adversarial
training~\cite{Kurakin16AdvTrain}).


==> tables/architectures.tex <==
\begin{table*}[htp]
\begin{center}
\small
  \tabcolsep=0.11cm
  \begin{tabular} { m{2cm} m{11cm} }
	\toprule
	% heading
	\emph{Model} & \emph{Architecture} \\ \midrule
	% content
	%%
	\gen{} (generator) & 
		{\footnotesize
			$\mathit{FC} (25\times 7040) \rightarrow$
			$\mathit{RB} \rightarrow$
			$\mathit{Reshape} (200, 4, 11) \rightarrow$
			$\mathit{Deconv} \rightarrow$
			$\mathit{RB} \rightarrow$
			$\mathit{Deconv} \rightarrow$
			$\mathit{RB} \rightarrow$
			$\mathit{Deconv} \rightarrow$
			$\mathit{RB}$
			$\rightarrow \mathit{Deconv} \rightarrow$
			$\mathit{tanh}$
		}\\
%		\includegraphics[height=1in]{figures/arch-gen.pdf}\\
%	%%
	\discrim{} (discriminator) & 
		{\footnotesize
			$\mathit{Conv} \rightarrow$
			$\mathit{LReLu} \rightarrow$
			$\mathit{Conv} \rightarrow$
			$\mathit{LrB} \rightarrow$
			$\mathit{Conv} \rightarrow$
			$\mathit{LrB} \rightarrow$
			$\mathit{Conv} \rightarrow$
			$\mathit{LrB} \rightarrow$
			$\mathit{Flatten} \rightarrow$
			$\mathit{FC} (7040\times 1)$
			$\rightarrow \mathit{Sigmoid}$
		}\\[3pt]
%		\includegraphics[height=1in]{figures/arch-discrim.pdf}\\[3pt]
%	%%
	\vggS & 
		{\footnotesize
			$\mathit{FC} (4096\times 10) \rightarrow$
			$\mathit{softmax}$}\\
%		\includegraphics[height=1in]{figures/arch-vgg10.pdf}\\
	\vggL & 
		{\footnotesize
			$\mathit{FC} (4096\times 143) \rightarrow$
			$\mathit{softmax}$ 
		}\\
%		\includegraphics[height=1in]{figures/arch-vgg143.pdf}\\
	\openfaceS &
		{\footnotesize
			$\mathit{FC} (128\times 12) \rightarrow$
			$\mathit{tanh} \rightarrow$
			$\mathit{FC} (12\times 10) \rightarrow$
			$\mathit{softmax}$
		}\\
%		\includegraphics[height=1in]{figures/arch-openface10.pdf}\\
	\openfaceL &
		{\footnotesize
			$\mathit{FC} (128\times 286) \rightarrow$
			$\mathit{tanh} \rightarrow$
			$\mathit{FC} (286\times 10) \rightarrow$
			$\mathit{softmax}$ 
		}\\[3pt]
%		\includegraphics[height=1in]{figures/arch-openface143.pdf}\\[3pt]
%	%%
	Detector &
		{\footnotesize
			$\mathit{Conv} \rightarrow$
			$\mathit{RB} \rightarrow$
			$\mathit{MP} \rightarrow$
			$\mathit{Conv} \rightarrow$
			$\mathit{RB} \rightarrow$
			$\mathit{Conv} \rightarrow$
			$\mathit{RB} \rightarrow$
			$\mathit{FC} (196\times 2) \rightarrow$
			$\mathit{softmax}$
		}\\
%		\includegraphics[height=1in]{figures/arch-detector.pdf}\\
	\bottomrule
	\end{tabular}
	\caption{Architectures of the neural-networks used in this work.
	For the OpenFace and VGG \dnn{}s, we only report the layers
	we added for the base, feature extraction, \dnn{}s.
	$\mathit{Conv}$ refers to convolution,
	$\mathit{Deconv}$ to deconvolutional (a.k.a, transposed convolution),
	$\mathit{FC}$ to fully-connected layer,
	$\mathit{Flatten}$ to vectorization of matrices,
	$\mathit{LrB}$ to batchnorm followed by a leaky rectified-linear layer,
	$\mathit{LReLu}$ to leaky rectified-linear layer,
	$\mathit{MP}$ to max-pooling layer,
	$\mathit{RB}$ to batchnorm followed by a rectified-linear layer,
	and $\mathit{tanh}$ to hyperbolic tanget.
	All convolutions and de-convolutions in \gen{} and \discrim{} use $5\times 5$
	filters, and have strides and paddings of two.
	The detector's convolutions use $3\times 3$ filters, have strides of two, and
	padding of one. The detector's $\mathit{MP}$ layer has a $2\times 2$ window size
	and a stride of two.} 
\label{tab:dnn_archs}
\end{center}
\end{table*}



